DepsRAG: Towards Agentic Reasoning and Planning for Software Dependency Management

In the era of Large Language Models (LLMs) with their advanced capabilities, a unique opportunity arises to develop LLM-based digital assistant tools that can support software developers by facilitating comprehensive reasoning about software dependencies and open-source libraries before importing them. This reasoning process is daunting, mandating multiple specialized tools and dedicated expertise, each focusing on distinct aspects (e.g., security analysis tools may overlook design flaws such as circular dependencies, which hinder software maintainability). Creating a significant bottleneck in the software development lifecycle. In this paper, we introduce DepsRAG, a multi-agent framework designed to assist developers in reasoning about software dependencies. DepsRAG first constructs a comprehensive Knowledge Graph (KG) that includes both direct and transitive dependencies. Developers can interact with DepsRAG through a conversational interface, posing queries about the dependencies. DepsRAG employs Retrieval-Augmented Generation (RAG) to enhance these queries by retrieving relevant information from the KG as well as external sources, such as the Web and vulnerability databases, thus demonstrating its adaptability to novel scenarios. DepsRAG incorporates a Critic-Agent feedback loop to ensure the accuracy and clarity of LLM-generated responses. We evaluated DepsRAG using GPT-4-Turbo and Llama-3 on three multi-step reasoning tasks, observing a threefold increase in accuracy with the integration of the Critic-Agent mechanism. DepsRAG demo and implementation are available: https://github.com/Mohannadcse/DepsRAG.

==> abstract.tex <==
\begin{abstract}
Managing software dependencies is a crucial maintenance task in software development. It is becoming a rapidly growing research field, especially in light of the significant increase in software supply chain attacks. Specialized expertise and substantial developer effort are required to fully comprehend dependencies and reveal hidden properties (e.g., number of dependencies, dependency chains, depth of dependencies).
Recent advancements in Large Language Models (LLMs) allow the retrieval of information from various data sources for response generation, thus providing a new opportunity to uniquely manage software dependencies. To highlight the potential of this technology, we present~\tool, a proof-of-concept Retrieval Augmented Generation (RAG) approach that constructs direct and transitive dependencies of software packages as a Knowledge Graph (KG) in four popular software ecosystems. \tool can answer user questions about software dependencies by \textit{automatically} generating necessary queries to retrieve information from the KG, and then augmenting the input of LLMs with the retrieved information. \tool can also perform a Web search to answer questions that the LLM cannot directly answer via the KG. We identify tangible benefits that~\tool can offer and discuss its limitations.
\footnote{\tool demo and implementation are available here: 
\url{https://shorturl.at/npyIZ}.}
% demo and implementation are available here
\end{abstract}

==> approach.tex <==
\section{\tool: Multi-Agent System for Dependency Management}

\begin{figure}[tb!]
    \raggedright  \includegraphics[width=\linewidth,keepaspectratio]{images/DepsRAG_Arch.pdf}
    % \vspace{-0.7cm}
    \caption{\tool high-level agentic architecture}
    \label{fig:depRAG_arch}
\end{figure}

This section describes the architecture of \tool, a chatbot for automatically constructing software dependencies as a knowledge graph and then answering use's queries, expressed in natural language, about the dependency graph. We first give a high-level outline of the objectives of the key sub-tasks in Section~\ref{sec:obj}, and delve into their implementation details in Section~\ref{sec:interaction}
- \ref{}. See Figure~\ref{} for an illustrative depiction of the overall pipeline.

We underscore that the development of a multi-agent RAG system specifically designed for comprehending and managing software dependencies presents significant challenges. This process requires careful consideration of several key factors: (a) the intricate hierarchical structure of software dependencies, which poses difficulties for standard RAG methods when applied naively; (b) the inherent brittleness of LLMs, including issues such as instruction deviation, hallucination, and generation of inaccurate or erroneous outputs; and (c) potential risks in inter-agent communication, such as infinite loops, fixed points, and deadlocks, which necessitate careful orchestration to ensure system robustness.

\tool consists of two retrievers whose responses augment the prompt with additional information, as illustrated in Figure~\ref{fig:depRAG_arch}. 
% The following is a description of these retrievers:
\begin{itemize}
    \item \textbf{KG Retriever}. This component retrieves information from the KG. It translates the user's question in natural language to the query language used by the KG, executes the query, and sends back the response to \tool. This component has two tools to perform these tasks: GraphSchemaTool and CypherQueryTool. The former tool provides the KG schema to \tool, which is needed to generate the query with the right entity names and relationships. The other tool receives the query generated by the LLM, executes it, and returns the response.
    \item \textbf{Web Search Retriever}. This component acts as a failover mechanism and answers when no answer is obtained from the KG. It also provides answers beyond the scope of the KG. For example, the user could ask \tool if one of the packages in the dependency KG is vulnerable. This component leverages WebSearchTool to perform a Web search and retrieve top-3 outcomes, and then the LLM can extract the most relevant results.
\end{itemize}

\noindent
Prompt~\ref{myPromptLabel} outlines the prompt used by~\tool. This prompt consists of three parts. \circled{$\textrm{R}$} defines the role of \tool. \circled{$\textrm{p}_1$} and \circled{$\textrm{p}_2$} describe the instructions for the two phases of \tool:
\begin{itemize}
    \item \textbf{\circled{$\textrm{p}_1$} Dependency KG Construction}. The user provides the name of the package, the version, and the ecosystem, and then \tool constructs the dependency graph following the graph schema illustrated in Figure~\ref{fig:schema}. According to this schema, the nodes in the KG belong to the entity Package, which has only two properties, the package name and version. For entity relationships, there is only one relation ``depends\_on''. \tool leverages ConstructKGTool for constructing the KG. Suppose the user did not provide the version and ecosystem of the package. In this case, \tool triggers the Web Search Retriever to find the version and ecosystem based on the provided package name. Figure~\ref{fig:phase1_illustration} illustrates the workflow of this phase to construct the dependency graph of the OpenAI package in the PyPI ecosystem.
    
    \item \textbf{\circled{$\textrm{p}_2$} QA Chatting.} After constructing the dependency KG for the provided package name, the user can ask any questions about the KG. In this phase, the KG Retriever and Web Search Retriever are employed to augment user questions with additional information. Figure~\ref{fig:phase1_illustration} illustrates the workflow of this phase. 
\end{itemize}

% \vspace{-0.2cm}
\prompt[myPromptLabel]{Prompt~\thepromptbox: \tool Instructions}{
\circled{$\textrm{R}$} \textbf{Define LLM Role}: {\it You are an expert in software dependency graphs and analyzing them using Neo4j.} 
\newline
\circled{$\textrm{p}_1$} \textbf{Phase-1 Task Instructions}: {\it FIRST, I'll give you the name of the package that I want to analyze.
% \newline
THEN, you can use the "WebSearchTool" to find out information about a package, such as version number and package type (PyPI, NPM, Cargo, or GO). If you cannot get this information, ask me and I can tell you.
% \newline
DON'T forget to include the package name in your questions. 
After receiving this information, ensure to get the package version type. 
% \newline
THEN ask the user if they want to construct the dependency graph, and if so, use "ConstructKGTool" to construct the dependency graph. Otherwise, say "Could not retrieve package type or version" and NO\_ANSWER.}

% \newline

\circled{$\textrm{p}_2$} \textbf{Phase-2 Task Instructions}: {\it After constructing the dependency graph successfully, you will have access to the Neo4j graph database, which contains the dependency graph. You will try your best to answer my questions. Note that:
\newline
    1. You can use "GraphSchemaTool" to get node labels and relationships in the dependency graph. \newline
    2. You can use "CypherQueryTool" to get relevant information from the graph database. I will execute this query and send you the result. Make sure your queries comply with the database schema. \newline
    3. Use the "WebSearchTool" to get information if needed. \newline
    4. To show the dependency graph, use  "VisualizeKGTool".}
}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.65\linewidth,keepaspectratio]{images/schema.pdf}
    \vspace{-0.6cm}
    \caption{Dependency KG Schema consisting of a single entity with two attributes, ``name'' and ``version'', and one relation.}
    \label{fig:schema}
\end{figure}

\noindent
Finally, we equipped \tool with utility tools, such as VisualizeKGTool, which is used to visualize the KG. Table~\ref{table:toolSummary} summarizes the tools used by \tool. 

\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.85\linewidth,keepaspectratio]{images/depRAG_phase_1.pdf}
    % \vspace{-0.4cm}
    \caption{Phase-1 of \tool in action.}
    \label{fig:phase1_illustration}
\end{figure}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.85\linewidth,keepaspectratio]{images/depRAG_phase_2.pdf}
    % \vspace{-0.4cm}
    \caption{Phase-2 of \tool in action.}
    \label{fig:phase2_illustration}
\end{figure}

\begin{comment}
\begin{table}[]
\centering
\caption{Summary of tools used by \tool.}
\vspace{-0.4cm}
\scalebox{0.82}{
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|l|}{\textbf{Tool Name}} & \textbf{Retriever} & \multicolumn{1}{l|}{\textbf{Purpose}} \\ \hline
GraphSchemaTool & KG & Obtain the KG schema \\ \hline
CypherQueryTool & KG & \begin{tabular}[c]{@{}l@{}}Receive the generated query, execute it, \\ and return the query result\end{tabular} \\ \hline
WebSearchTool & Web Search & \begin{tabular}[c]{@{}l@{}}Perform web search, receive top-3 results, \\ and return the most relevant\end{tabular} \\ \hline
ConstructKGTool & N/A & Construct the KG \\ \hline
VisualizeKGTool & N/A & Visualize the KG \\ \hline
\end{tabular}
}
\label{table:toolSummary}
\end{table}
\end{comment}


\begin{table}[]
\centering
\caption{Summary of tools used by \tool.}
\vspace{-0.4cm}
\scalebox{0.8}{
\begin{tabular}{lll}
\toprule
\textbf{Tool Name} & \textbf{Retriever} & \textbf{Purpose} \\ \midrule
GraphSchemaTool & KG & Obtain the KG schema \\ 
CypherQueryTool & KG & \begin{tabular}[c]{@{}l@{}}Receive the generated query, execute it, \\ and return the query result\end{tabular} \\ 
WebSearchTool & Web Search & \begin{tabular}[c]{@{}l@{}}Perform Web search, receive top-3 results, \\ and return the most relevant\end{tabular} \\ 
ConstructKGTool & N/A & Construct the KG \\ 
VisualizeKGTool & N/A & Visualize the KG \\ \bottomrule
\end{tabular}
}
\label{table:toolSummary}
\end{table}





==> implementation.tex <==
\section{Implementation}
Our implementation of \tool was realized using Python 3.11, with the assistance of Langroid~\cite{langroid}. This framework supports the development of multi-agent LLMs and enables seamless integration with a variety of LLMs. Moreover, Langroid can orchestrate the interaction between LLMs and tools. Finally, Langroid contains built-in tools to facilitate the development of RAG applications to perform web search and access Neo4j, a graph database management system. 

To obtain the dependencies for the provided project and construct the dependency KG, we used \texttt{deps.dev} API, a service developed and hosted by Google to help developers better understand the structure, construction and security of open source software packages. This API is used by prior work~\cite{rahman2024characterizing,linuntrustide} to characterize and analyze dependencies.
This service repeatedly examines sites such as GitHub, NPM, and PyPI to find up-to-date information about open source software packages and thus generating a comprehensive list of direct and transitive dependencies, which are constantly updated. \tool receives a JSON response from the \texttt{deps.dev} API. This JSON file contains a list of dependencies of the provided package. Then the tool \texttt{ConstructKGTool} propogates the data in the JSON file to build the dependency KG. 

The experiments were carried out on a system equipped with a 2.3 GHz Quad-Core Intel Core i7 processor, 32 GB of RAM, and running macOS Sonoma.

==> preliminaries.tex <==
\section{Preliminaries on LLM-based Agents}
Despite the impressive capabilities of today's LLMs, they face limitations such as brittleness, non-determinism, limited context windows, inference costs, and latency~\cite{bommasani2023holistic}. As a result, one cannot rely on LLMs to handle complex tasks with only high-level instructions. To fully utilize LLMs in complex applications, tasks must be broken down into smaller subtasks, each managed by distinct LLM conversations, each with specific instructions, states, and data. This naturally introduces the concept of an agent, an LLM-powered entity dedicated to handling a specific sub-task~\cite{MALADE}.

\subsection{Agentic LLM Applications}
\textbf{Agents.} An agent is responsible for a specific aspect of a task, acting essentially as a message transformer. In code, an agent is typically represented as a class encapsulating an interface to an LLM, along with optional tools and external data (e.g., a vector database). Agents communicate by exchanging messages, similar to the actor model in programming~\cite{actor}. For practical applications, agents can trigger actions (e.g., API calls, computations) and access external data, facilitated by tools and RAG.

\noindent
\textbf{Tools, also known as functions or plugins.} Tools allow LLMs to trigger external actions beyond generating text. While free-form text is useful for descriptions, summaries, or agent queries, structured outputs are needed for actions like API calls, code execution, or database queries. In such cases, the LLM produces a structured response, typically in JSON format, specifying necessary details like code or query parameters. The LLM uses a tool when generating such structured responses, and a tool handler is defined to execute the corresponding action when recognized in the LLM’s output.

\noindent
\textbf{Retrieval-Augmented Generation (RAG).}
Utilizing an LLM in isolation presents two primary limitations: (a) its responses are confined to the knowledge available at the time of pre-training, making it incapable of addressing questions related to private sources (such as databases or documents) or post-training information, and (b) it cannot verify the correctness of its responses. RAG mitigates these challenges by generating answers based on specific documents or data while also providing source references for validation. When an LLM receives a query $Q$ in the RAG process, it retrieves a set of $k$ most relevant pieces of data $D = {d_1, d_2, \dots, d_k}$ from a database store. The query is then reformulated into a new prompt: ''Given the following data: $[d_1, d_2, \dots, d_k]$, provide an answer to this question: $Q$, based ONLY on these data, and indicate which data support your answer.'' 

\noindent
\textbf{Multi-Agent Orchestration}
An orchestration mechanism is critical to ensure task progress, manage message flow, and handle deviations from instructions. This work adopts a multi-agent programming approach, where agents are first-class entities interacting via message exchange. These messages manage and facilitate the interactions between agents (i.e., inter-agent communication) and within individual agents (i.e., intra-agent communication between tools within the agent itself). 
This functionality is commonly managed by frameworks designed for developing applications with Large Language Models (LLMs). Frameworks such as Langroid~\cite{langroid} and Langchain~\cite{langchain} provide robust mechanisms for message routing and task delegation. In this work, we utilize the Langroid framework, which offers a streamlined orchestration mechanism to efficiently manage user interactions, tool integrations, and sub-task delegation. Langroid's orchestration is encapsulated within the Task class, which wraps an agent and initiates a task through the invocation of its \textsc{run} method. The Task maintains a ``current pending message'' (CPM) that is processed by one of its responders, which can include the agent’s response methods or the run methods of sub-tasks. The run method iterates through a sequence of ``steps'' until a termination condition for the task is met. During each step, the system seeks a valid response to the CPM by evaluating all available responders, and the CPM is updated accordingly as the task progresses.

In \tool, we developed a suite of advanced routing tools and a critic agent, built on top of the Langroid framework, to enhance reasoning and comprehension within software dependency environments. These extensions are designed to improve the framework’s ability to handle complex dependency structures and facilitate more accurate analysis and decision-making processes.

==> questions.tex <==
\begin{table*}[]
\centering
\caption{Comparing the performance of the considered LLMs to answer graph properties questions about the dependency graph for the TensorFlow NPM package illustrated in Figure~\ref{fig:tensorflow}.}
\vspace{-0.3cm}
\scalebox{0.7}{
\begin{tabular}{|p{3cm}|c|c|p{6cm}|l|p{6.5cm}|l|}
\hline
\textbf{Question} & \textbf{\# steps} & \textbf{Query trials} & \multicolumn{1}{c|}{Cypher Query} & \multicolumn{1}{c|}{LLM} & \multicolumn{1}{c|}{Response} & \multicolumn{1}{c|}{Correct Response} \\ \hline
\multirow{2}{*}{\makecell{what's the depth of the\\dependency graph?}} & 1 & 0 & MATCH   p=(pkg:Package)-[:DEPENDS\_ON*]->(:Package) RETURN length(p) AS Depth ORDER BY Depth DESC LIMIT 1 & GPT-4-Turbo & The depth of the dependency graph is 13 levels deep. This means that the longest chain of dependencies from one package to another spans 13 levels. & yes \\ \cline{2-7} 
 & 1 & 1 & MATCH   p=(n)-[*]->() RETURN max(length(p)) as depth & Llama-3 & The depth of the   dependency graph is 13 & yes \\ \hline
 \multirow{2}{*}{\makecell{Are there cycles in the\\dependency graph?}} & 1 & 0 & MATCH   (pkg:Package)-[:DEPENDS\_ON*]->(pkg2:Package) WHERE pkg.name = pkg2.name RETURN pkg.name AS PackageWithCycle & GPT-4-Turbo & \begin{tabular}[c]{@{}l@{}}\makecell[l]{Yes, there are cycles in the dependency graph.\\The following packages have been identified\\as having cyclic dependencies:\\      \\      - `es5-ext`\\      - `es6-iterator`\\      - `es6-symbol`\\      - `esniff`\\      - `event-emitter`\\      \\      These packages appear to depend on\\themselves through a chain of dependencies,\\which is indicative of a cyclic dependency}.\end{tabular} & yes \\ \cline{2-7} 
  & 1 & 0 & MATCH (n)-[:DEPENDS\_ON]->(m) WHERE id(n) < id(m) RETURN count(*) as cycle\_count & Llama-3 & Yes, there are cycles in the dependency graph & yes \\ \hline
 \multirow{2}{*}{\makecell{how many path chains \\in the dependency\\graph?}} & 1 & 0 & MATCH   p=(pkg:Package)-[:DEPENDS\_ON*]->(:Package) WHERE pkg.name = 'tensorflow'   AND pkg.version = '0.7.0' RETURN count(p) AS pathCount & GPT-4-Turbo & There   are 133 path chains in the dependency graph for the TensorFlow NPM package   version 0.7.0 & yes \\ \cline{2-7} 
  & 1 & 2 & MATCH (n)-[r:DEPENDS\_ON]->() RETURN COUNT(DISTINCT r) AS num\_paths & Llama-3 & It looks like there are 44 path chains in the dependency graph & no \\ \hline
\multirow{2}{*}{\makecell{What's the density of\\the dependency graph?}} 
& 2 & 0 & \begin{tabular}[c]{@{}l@{}}\makecell[l]{Step-1: MATCH (n) RETURN count(n) as\\ nodeCount}\\ \makecell[l]{Step-2: MATCH ()-[r]->() RETURN count(r) as\\ relationshipCount}\end{tabular} & GPT-4-Turbo & \begin{tabular}[c]{@{}l@{}}\makecell[l]{To calculate the density of the graph,\\we use the formula:
    \text{Density} = $\frac{E}{N(N-1)}$ \\where $E$ is the number of edges (relationships)\\and $N$ is the number of nodes (vertices) in the\\graph.
    Given that we have: $N = 25$ nodes\\
    and $E = 44$ edges
    \\
    The density $D$ of the graph is:
    \\
    $D = \frac{44}{25(25-1)}$
    $D = \frac{44}{600}$
    $D = 0.0733$
    \\
    The density of the graph is approximately\\ 0.0733. This indicates that out of all possible\\connections that could exist in the graph,\\around 7.33\% are actually present.}
\end{tabular} & yes \\ \cline{2-7}

& 2 & 0 & \begin{tabular}[c]{@{}l@{}}\makecell[l]{MATCH (p:Package) RETURN count(p) AS \\num\_packages}\\ \makecell[l]{MATCH ()-[r:DEPENDS\_ON]->() \\RETURN count(r) AS num\_dependencies}\end{tabular} & Llama-3 & \begin{tabular}[c]{@{}l@{}}Now that I have the number of nodes (packages)\\and edges (dependencies), I can calculate the\\density of the graph.\\ The density of the graph is calculated as the ratio\\of the number of edges to the maximum possible\\number of edges. In an undirected graph, the\\maximum possible number of edges is $n(n-1)/2$,\\where $n$ is the number of nodes.\\ In this case, the number of nodes (packages) is 25,\\and the number of edges (dependencies) is 44.\\ The maximum possible number of edges is\\$25(25-1)/2 = 300$.\\The density of the graph is then $44/300 = 0.1467$.\\ So, the density of the graph is approximately 0.147.\end{tabular} & no \\ \hline


\end{tabular}
}
\label{tab:questions}
\end{table*}
